Automated Discovery of Adaptive Attacks on Adversarial Defenses

Reliable evaluation of adversarial defenses is a challenging task, currently limited to an expert who manually crafts attacks that exploit the defense's inner workings or approaches based on an ensemble of fixed attacks, none of which may be effective for the specific defense at hand. Our key observation is that adaptive attacks are composed of reusable building blocks that can be formalized in a search space and used to automatically discover attacks for unknown defenses. We evaluated our approach on 24 adversarial defenses and show that it outperforms AutoAttack, the current state-of-the-art tool for reliable evaluation of adversarial defenses: our tool discovered significantly stronger attacks by producing 3.0\%-50.8\% additional adversarial examples for 10 models, while obtaining attacks with slightly stronger or similar strength for the remaining models.

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Our main contribution is to automate the adaptive attacks by searching through a search space formulated by existing techniques. The quantitative results are supported by Table 1 in the evaluation.}
  \item Did you describe the limitations of your work?
    \answerYes{They are mentioned in the last paragraph in conclusion section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In this paper, an approach to improve the evaluation of adversarial defenses by automatically finding adaptive adversarial attacks is proposed and evaluated. In general, such tool can be used both in a beneficial way by the researches developing adversarial defenses, as well as, in a malicious way by an attacker trying to break existing models. In both cases, the approach is designed to improve empirical model evaluation, rather than providing verified model robusness, and thus is not indended to provide formal robustness guarantees for safety critical applications.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Our theoretical result is the time bound analysis and the assumptions are stated in Appendix A.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Included in Appendix~A.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is provided as anonymous github repository. All the instructions are included in README.md}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All hyperparameters of the search are included in evaluation section, and the search space is defined in Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Unfortunately, given the large number of experiments all the results of our tool are reported from a single run. Whenever possible, we compared to the results reported in prior works (AutoAttack, RobustBench) and we were able to replicate the results within a very small margin of error ($\leq 0.3$ robust accuracy in Table~1).}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We use single GTX2080Ti GPU as described in the evaluation.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited the dataset, the libraries, and the models we use.}
  \item Did you mention the license of the assets?
    \answerNo{We will release our tool and codebase using permissible Apache-2.0 License. However, we did not mention this explicitly in the paper. Likewise, the licenses of prior works are included in their respective public repostories, but not explicitly stated in the paper.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide an anonymized github repository containing our tool and scripts to replicate the experiments.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{we use publicly available CIFAR-10.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{we use publicly available CIFAR-10.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> figures/loss_functions.tex <==


\begin{figure}[t]
\centering
\begin{tikzpicture}[trim left=-12em]

\node at (-1.2,0) {
\begin{minipage}{0.4\textwidth}
\begin{equation*}%\eqlabel{standard_ml}
\textstyle
\ell_{\texttt{CrossEntropy}} = - \sum_{i = 1}^{K} y_i \log(Z(x)_i)
\end{equation*}
\end{minipage}
};

\node at (0,-0.9) {
\begin{minipage}{0.4\textwidth}
\begin{equation*}%\eqlabel{standard_ml}
\displaystyle
\ell_{\texttt{HingeLoss}} = \max(- Z(x)_y + \max_{i \neq y} Z(x)_i, -\kappa)
\end{equation*}
\end{minipage}
};

\node at (-2.5, -1.45) {
\scriptsize \cite{CandW}
};

\node at (-1.2,-2.0) {
\begin{minipage}{0.4\textwidth}
\begin{equation*}%\eqlabel{standard_ml}
\displaystyle
\ell_{\texttt{L1}} = - Z(x)_y
\end{equation*}
\end{minipage}
};

\node at (-0.0,-3.1) {
\begin{minipage}{0.4\textwidth}
\begin{equation*}%\eqlabel{standard_ml}
\displaystyle
\ell_{\texttt{DLR}} = - \frac{Z(x)_y - \max_{i \neq y} Z(x)_i}{Z(x)_{\pi_1} - Z(x)_{\pi_3}}
\end{equation*}
\end{minipage}
};

\node at (-2.5, -3.55) {
\scriptsize \cite{croce2020reliable}
};

\node at (-1.4,-4.1) {
\begin{minipage}{0.4\textwidth}
\begin{equation*}%\eqlabel{standard_ml}
\displaystyle
\ell_{\texttt{LogitMatching}} = \norm{Z(x') - Z(x)}_2^2
\end{equation*}
\end{minipage}
};

\end{tikzpicture}
\vspace{-0.2em}
\caption{Loss functions used as part of the loss search space $\sL$. }
\label{loss_functions}
\end{figure}

==> overview.tex <==
\section{Meta-Attack System Definition}

Figure \ref{fig:overview} gives an overview of the meta-attack system which is denoted as $\gM$. There are three search spaces in meta-attack: the network transformation space $\sG$, attack search space $\sS$, and loss function search space $\sL$. $\gM$ takes model $f$ and dataset $\mD$ as inputs, and outputs the network $g^{*}$ from $\sG$ and attack $s^{*}$ from $\sS \times \sL$. This is denoted as: 

\begin{equation}
\label{ma_signature}
g^{*}, s^{*} = \gM(f,\mD) \text{, where } g^{*} \in \sG, s^{*} \in \sS \times \sL
\end{equation}

Here, $g^{*}$ is referred as attack network meaning $s^{*}$ is performed on $g^{*}$ instead of $f$. $g^{*}$ is only used when applying the attack, whereas $f$ network is used to check if the generated examples are adversarial. 

For the meta-attack system implementation, we separate the network processing phase and the attack search phase. We first find the attack network $g^{*}$ during the network processing phase, and then we search the attack $s^{*}$ using $g^{*}$. The search space will be presented in section 4, and the search algorithm will be presented in section 5. 


\subsection{Meta-attack Specification}

The specification of meta-attack is to define the signature of input network $f$ and all the parameters inside of $\gM$. When specified, $\gM$ is a function with in equation \ref{ma_signature}. 

A threat model specifies the conditions under which a defense is designed to be secure and the precise security guarantees provided \cite{carlini2019evaluating}. It is important to specify the threat model in $\gM$ in order to meaningfully test the defenses. 

To specify $\gM$. We need to define the input output dimension constraints (1), threat model (2-5), the search space (6), and the search algorithm (7). The specification used in the experiments are shown in italic. 

% A threat model contains four aspects. Firstly, there is an adversarial goal. It may be mis-classification, or targeted mis-classification, or other criteria in different tasks. Secondly, the constraint of adversarial examples needs to be defined. The mostly used constraint is L-p norm with disturbance $\epsilon$, but it can also be spatial transformation \cite{xiao2018spatially} or physical realizable \cite{wu2019defending}. Thirdly, the computation constraint of the adversarial model needs to be defined. The constraint can be the limited number of queries to the network or some time limit. Fourthly, the adversarial knowledge on the model needs to be specified. This can be white box, where the attacker has full access to the model. It can also be blackbox with varies access levels, for example accessing all logits, top class probabilities only and so forth. 

\begin{enumerate}
    \item The input space $\sX$ and output space $\sY$. All input network $f$ has the signature: $f: \sX \rightarrow \sY$. \textit{CIFAR10: $\sR^{32\times32\times3} \rightarrow \sR^{10}$}
    \item The adversary goal defined by a criterion function $C$. \textit{Misclassification}
    \item The adversary computation capability defined by time or number of queries constraint denoted by $T_{c}$. \textit{Defined by the wall time per sample}
    \item The adversary disturbance capability is defined by the type of distance measurement (e.g. L-p norm) and the budget of the disturbance $\epsilon$. \textit{L-inf norm, $\epsilon=4/255$ or $\epsilon=8/255$}
    \item The adversary knowledge of the input network (e.g. whitebox, blackbox with logit access, etc.) \textit{Whitebox}
    \item The network transformation space $\sG$, attack search space $\sS$, loss search space $\sL$. \textit{Details in section 4}
    \item The search algorithm along with its parameters. \textit{Details in section 5}
\end{enumerate}

This work uses this specification on image classification, but the idea of meta-attack can be generalized to other domains (e.g. NLP, RL) and on other threat models.  


\subsection{Preliminaries} 

Here defines some other notations used in the paper. 

\paragraph{Dataset} 
An input image and its label are denoted as $\vx$ and $y$ respectively. The dataset $\mD$ is defined as the set of image and label pair ($(\vx, y) \in \mD$). 

\paragraph{Input model} 
$\sX$ is the vector space of input image $\vx \in \sX$. $\sY$ is the space of vectors with the dimension of the number of classes, and in the formulation we treat integer labels as vectors. $\gM$ only admits models with signature $\sX \rightarrow \sY$, and the set of all such models are denoted as $\sF$. Any input network $f$, $f \in \sF$, can be expressed as $\vz=f(\vx)$, where $\vz$ denotes the class probability or logit vector. 

\paragraph{Loss function} Loss function takes the prediction and the label as inputs and has the signature of $L:\sY, \sY -> \sR$. 

\paragraph{Attacks in meta-attack} The attack $s$ admissible to the $\gM$ has the signature $s:\sF \times \sX \rightarrow \sX$, and it is subjective to the threat model defined in $\gM$. Attack $s$ can also be expressed as $\vx'=s(f,\vx)$ where $\vx'$ is the adversarial image candidate generated by attack $s$. 

\paragraph{Criterion function} The criterion function $C$ has the signature of $C:\sF \times \sX \times \sY \rightarrow \{0,1\}$. It can be expressed as $c=C(f,\vx',y)$ with $c=1$ denoting the attack is successful and $c=0$ otherwise. 

% The criterion function for misclassification is shown in equation \ref{misclassification}. 

%Note that the formulation of criterion function is general and other criterion like targeted misclassification can be formulated similarly. 
% The attack success score is defined as $c=C(f,\vx',z)$ with $c=1$ denoting the attack is successful and $c=0$ otherwise. Here $C$ is the attack success criterion function, $z$ is the criterion. In misclassification, $z=y$, and in targeted classification, $z$ is the specified targeted class. 

%\begin{equation}
%    \label{misclassification}
%     C_{\texttt{misclassification}}(f, \vx, y) =
%  \begin{cases}
%    1  & \quad \text{if } z(=f(\vx)) \neq y\\
%    0  & \quad \text{otherwise}
%  \end{cases}
%\end{equation}

\paragraph{Detector formulated in Criterion function} A detector model is a binary classifier that is designed to differentiate between real and adversarial examples. %cite
In this work, detector is formulated within the criterion function $C$, where the detector needs to classify $\vx'$ as real example for it to be considered adversarial. This formulation of the detector can be classified as zero knowledge adversarial \cite{biggio2013evasion}. For future work, MA can be extensions to include the knowledge of detectors. 

%, which contains both the previously defined misclassification criterion $C_{1}$ and the detector $C_{2}$. We define the output of $C_{1}$ and $C_{2}$ to be $c_{1}$ and $c_{2}$ respectively. We define $c_{2}=0$ if the detector classifies it as adversarial and $c_{2}=1$ otherwise. The final output of $C$, can be defined as $c=c_{1} \land c_{2}$. This formulation of the detector can be classified as zero knowledge adversarial \cite{biggio2013evasion} since the attack is not aware of the detector. There can be alternative formulations to include the knowledge of detectors. 

\paragraph{Note on Randomness}  All function expressions can have random seed in the formulation if they have random component. To remove clutter, the random seed is not explicitly written, and the meaning of such expressions is to get a sample from the distribution of output. For example, the model $f$ can have randomized component, then $z=f(\vx)$ means a to draw a sample from the output distribution of $f(\vx)$ and assign it to $z$. The same reasoning applies to attack $s$ and criterion function $C$. 


\subsection{Objective of Meta-attack} 

\paragraph{Attack Success Rate (ASR)} 
Robustness of network, which refers to the percentage of samples that are correctly classified under an attack, is used as the criteria traditionally. Since this work emphasizes on the strength of attack, the new metric ASR is used. To calculate ASR, the samples with wrong predictions are removed first, and then ASR is the wrong prediction rate on adversarial samples generated by $s$ on the remaining samples. In this formulation, ASR ranges from $0\%$ to $100\%$ on any network. Formally, ASR is defined under a meta-attack system $\gM$ where adversarial disturbance capabilities and criterion function $C$ are defined. ASR is the metric to evaluate an attack $s$ on model $f$ and dataset $\mD$. We also add the attack network $g$ in the formulation. 

\begin{equation}
\label{ASR}
ASR_{\gM}(s,f,g,\mD)=\frac{\sum_{(x,y) \in \mD}{C(f,s(g,\vx),y) \land \neg C(f,\vx,y)}}{{\sum_{(x,y) \in \mD}\neg C(f,\vx,y)}}
\end{equation}

\paragraph{Objective Function} The objective of robustness evaluation is to minimize the robustness of the network, and this is equivalent to maximizing ASR. A constraint formulated under $\gM$ is that the attack needs to comply to the adversary computation capability $T_{c}$. The objective function of $\gM$ is to find $g^{*}, s^{*}$ such that:

\begin{equation}
\label{search_objective}
g^{*}, s^{*} = \argmax_{g \in \sG, s \in \sS \times \sL} ASR_{\gM}(s,f,g,\mD), \text{subjective to } T_{c}
\end{equation} 







==> search_impl.tex <==
\section{Search algorithm}

The search algorithm is shown as block diagram in figure \ref{fig:detail}. The search objective is defined in Equation \ref{search_objective}. The two search strategies are implemented separately and differently because network transformation search and attack search are expensive to search jointly and are very different in nature. The joint search of two search spaces can be a future research direction. 

\subsection{Network Transformation Search}
\begin{equation}
\label{network_objective}
    g^{*} = \argmax_{g \in \sG} ASR_{\gM}(s_{test},f,g,\mD_{test})
\end{equation}

\paragraph{Search Objective} The objective of network transformation stage is defined in \ref{network_objective}. At this stage, the evaluation is done by a test attack $s_{test}$, which is a budget version of APGD with untargeted CE loss. APGD is used for two reasons: this variant of PGD can be regarded as universal first order attack so that it can be representative \cite{madry2017towards}, and APGD is not as sensitive to parameters (especially step size) as PGD. Each attack network candidate is evaluated using $s_{test}$ on a large subset of $\mD$ called $\mD_{test}$ (set to be 2000 in the implementation).

%This transformation spaces of $\sT$ is defined to be $\sT_{B} \times \sT_{R}$ as shown in section 4.

\paragraph{Search Strategy} For the search, BPDA search is conducted first and then layer removal search. In each stage, exhaustive search strategy is used because the search space is small for the networks. 

\paragraph{Comment on Cost of Search} Comparing with Attack Search, this search spends a very small fraction of the time. However, as the search space expands, this cost should be evaluated. 


\subsection{Attack Search}

\begin{equation}
\label{attack_search_objective}
s^{*} = \argmax_{s \in \sS} ASR_{\gM}(s,f,g^{*},\mD')
\end{equation}


\paragraph{Search Objective} The objective is shown in \ref{attack_search_objective}, and the attack network $g^{*}$ is from the previous search stage. The goal is to find the sequence attack $s^{*}$ which consists of attack algorithm and loss function pairs. The sequence attack search is done iteratively for each attack algorithm and attack pairs.
 

\paragraph{Single Attack Search} There are three stages in the single attack search: dataset filtering, candidates selection, and Successive Halving (SHA). The first stage dataset filtering is to use the current list of attack $s'$ to filter out non-robust samples. During the first iteration, it filters out incorrect samples based on the criterion function $C$. The filtered dataset is denoted as $\mD'$. 

In the second stage, the two key components are the attack generation and evaluation. To generate attack candidates, TPE or random algorithms are used to sample attack from the search space $\sA \times \sL$, and each such sample is called a trial. The goal of attack evaluation is to compare the strength of the attacks and constrain the cost of the attack. ASR is the best measurement of the attack strength, but if the ASR is the same, we encourage stronger attack by using a surrogate loss. The evaluation is on a small randomly sampled subset of $\mD'$ denoted as $\mD_{eval}$. The score function is defined in Equation \ref{single_attack_search_score}, where $L$ is the average untargeted cross-entropy loss on $\mD_{eval}$, and $\lambda$ is a small constant so that $L$ is used as a tie breaker when ASR of two attacks are the same. If a trial violates the time constraint $T_{c}$, it will be discarded. In this stage, the two parameters are $|\mD_{eval}|$ denoted as $n_{s}$, and the number of trials denoted as $n_{t}$.

\begin{equation}
\label{single_attack_search_score}
  score =
    \begin{cases}
      ASR_{\gM}(s,f,g^{*},\mD_{eval}) - \lambda \times L & \\
      -\infty & \text{otherwise}
    \end{cases}       
\end{equation}

The third stage SHA \cite{li2018massively} is an iterative algorithm to address the trade-off between number of samples $n_{s}$ to run and the quality of evaluation. The first SHA iteration takes the top $n_{t}/\tau$ trials based on the scores, and evaluate on $n_{s} \times k$ samples. Here $\tau$ and $k$ are search parameters. This process runs iteratively until only one trial is left and the corresponding attack is selected as $a^{*}$. 


\paragraph{Sequence Attack Search} As shown figure \ref{fig:detail}, the sequence of attack search is iterating the single attack search, and the only change is the $\mD'$ used for the search. Each iteration an attack is found, it is added to the list of attack $s'$ which is used to filter out non-robust samples for the next iteration. The number of attack $n_{a}$ is a search parameter. 


\paragraph{Cost of Search} The runtime $T_{s}$ of attack search is bounded by the search parameters and time constraint $T_{c}$. If we ignore the small overhead of the algorithm and rounding error due to discretization, $T_{s}$ is bounded by: 

\begin{equation}
    T_{s} \le T_{c} \times n_{a} \times n_{t} \times n_{s} \times (\frac{1}{1-k/\tau})
\end{equation}

In the experiment setting (shown in Table \ref{parameters}), $\tau=4$ and $k=2$, $n_{s} \times n_{t} \times n_{a} \le 2*|\mD|$, then the cost of search is bounded by $4$ times the time budget of attacking the whole dataset $T_{c}*|\mD|$. Better evaluation result is expected to be achieved by increasing $n_{a}$, $n_{s}$, $n_{t}$ at the cost of longer search run time. 

\subsection{Limitations}
One major limitation of the approach is to include expensive attack efficiently. The expensive attacks (e.g. NES) require a magnitude longer $T_{c}$ for them to not time out, but this will impact on the search time. 

Another problem is the necessity of hand-craft search space and search parameters. The definition the range of parameters in the search space can affect the result, and the search result can be sensitive to the search parameters. 


==> search_space.tex <==
\section{Search Space Definition}

In meta-attack system $\gM$, the two search spaces are: network transformation space $\sG$ and the attack search space $\sS$. The attack search space further consists of algorithm search space $\sA$ and the loss search space $\sL$. 
%Since an attack consists of attack algorithm and loss function, the space of $\sS$ and $\sL$ are discussed together despite they are formulated independently. 

\subsection{Network Transformation Space}

%To define the network transformation search space, the computation model of $f$ is expressed as one of the corresponding directed acyclic graphs (DAG) $\gG$ (defined next), and then the allowed graph transformation operation $\sT(\gG)$ is defined. 

%DAG computational graph $\gG$ is defined as: $\gG = \langle V, W, E \rangle$, where $V$ denotes set of vertices to represent vectors, $W$ denotes set of vertices to represent operators, $E$ denotes the flow of the computation and $E \subseteq (V \times W) \cup (W \times V)$. Since operator vertex $w \in W$ can be defined at any granularity from a basic operator to large network, there are many valid graph representations of varying granularity for model $f$. We denote the space of all the possible DAG representation to be $\gF$, and we denote the relation as $\gG \in \gF$.
%PB{does this typecheck? $f$ is a network (a graph) whereas $\gG$ is also a graph. I dont think you mean that $\gG$ is a subgraph of $f$}. 

%In this formulation, backward path is modelled as a subgraph of $\gG$, denoted as $\gG_{b}=\langle V_{b}, W_{b}, E_{b} \rangle$. There are two special notes for $\gG_b$: Firstly, the loss function for back propagation is defined by attack not the DAG graph. Secondly, $\gG_b$ can be disconnected if the corresponding forward operator is non-differentiable or if the adversarial knowledge is blackbox. Concrete examples and more explanations can be found in Chapter 6, in figures \ref{fig:net4_graph} and \ref{fig:net6_forward}. 

%A graph transformation is a function $t\colon \gG=\langle V, W, E \rangle \rightarrow \gG'=\langle V', W', E' \rangle$ which transforms an input graph by adding, removing, replacing, or inserting operator vertices. $V$ and $E$ will be only changed according to $W'$. The graphical illustration of all the transformations are shown in figure \ref{fig:transformation}. When adding and removing an operator vertex, the operator vertex must have the same input output dimensions. When replacing an operator vertex, the new vertex must have the same signature as the replaced vertex. The insertion can only happen between two existing vector vertices in $\gG_b$, and the signature of the inserted operator must match the dimensions of the vectors. The space of all such transformation on $\gG$ is denoted as $\sT(\gG)$. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[trim=0 200 0 100,clip,width=1\linewidth]{figures/transformation.pdf}
%    \caption{The description of the allowed transformations. The same color of the vector vertices represent same vector dimensions}
%    \label{fig:transformation}
%\end{figure}

%The space $\sG$ is defined as applying transformation $t \in \sT(\gG)$, on any $\gG \in \gF$. 

The network $f$ can be expressed as a Directed Acyclic Graph (DAG) \cite{liu2019darts} with its vertices being operators (e.g. convolution, residual blocks, etc.) and edges being the connectivity. Network transformation is to transform the vertices, either backward function or both forward and backward function. 

The definition of $\sG$ consists two parts: computational graph definition, and transformations on the graph. In this work, we manually define the computational graph of $\gG$ for each input network. For transformations, two different transformations are considered: BPDA and vertex removal. We leave the automatic DAG interpretation and extensions to the current transformation space for future work. 

BPDA is to replace the backward graph of an operator. In implementation, the vertices subjective to this transformation are any operators with same input output dimensions and without a defined backward function. There are three candidates for BPDA forward substitution: identity functions, convolution layer with kernel size 1, and two layer convolutional layer with ReLU activation in between. The weights in the latter two candidates are learned through approximating the forward function, and they are trained on the full test dataset $\mD$ for 10 epochs. The transformations from the three candidates are denoted as $t_{B1}, t_{B2}, t_{B3}$ respectively, and we denote the transformation space to be $T_{B} = \{t_{B1}, t_{B2}, t_{B3}\}$. 

Layer removal is to removal an operator from the DAG. In implementation, as long as the operator's input and output dimensions are the same, it is a candidate for removal. The transformation space of such candidate consists of two choices: to remove or not to remove, denoted as $t_{R1}, t_{R0}$ respectively. The layer removal space on the candidate vertex is $T_{R} = \{T_{R1}, T_{R0}\}$. 

If there are $n$ BPDA candidates and $m$ removal candidates on a graph $\gG$, the multiplicative transformation space used in the search is $\sT = \prod_{i=1}^{n}T_{B}^{i} \times \prod_{j=1}^{m}T_{R}^{j}$. 

%\subsection{Attack Algorithm Search Space}

%In the attack search space, not only single attack is in the search space, but also a sequence of attacks. The reason for including this sequence of attack into the space is to let attack complement each other to achieve higher ASR. For any sequence of attack $s$ with length $n$, $n \in \sZ^{+}$, $s=[a_{1}, a_{2}, \ldots a_{n}]$, the semantics is to evaluate the attacks in order and return the first adversarial sample found as shown in Algorithm 1. The order in the sequence of the attacks matters as it affects the return of the adversarial image. It is worth noting that the notion of ensemble of attacks in AA is equivalent to this notion of sequence of attack. 
%
%\begin{algorithm}[tb]
%  \caption{Sequence of attacks}
%  \label{alg:seq_attack}
%\begin{algorithmic}
%  \STATE {\bfseries Input:} $g$, $\vx$, sequence attacks list $a$ with size n\; 
%  \STATE {\bfseries Output:} $\vx'$\;
%%   \REPEAT
%%   \STATE Initialize $noChange = true$.
%  \FOR{$i=1$ {\bfseries to} $n$}
%  	\STATE $\vx'$=$s[i](g, \vx)$\;
%    \IF{$C(\vx',g,y)$}
%      \STATE Return $\vx'$\;
%    \ENDIF
%    \ENDFOR
%  \STATE Return $\vx'$\;
%%   \UNTIL{$noChange$ is $true$}
%\end{algorithmic}
%\end{algorithm}

%To further define syntax of $\sS$, we use the grammar rules. 
%
%\begin{enumerate}
%    \item $\sS \rightarrow \sS;\sS| D(\sA)$
%    \item $D(\sA) \rightarrow Repeat(EOT(Randomize(\sA), m),n)$
%    \item $\sA \rightarrow a=PGD(param)|DF(param)|FAB(param)|...$
%\end{enumerate}
%
%$\sA$ is the space containing the attack algorithms along with the parameters. The algorithms include both the standard FGSM, PGD, C\&W, Deepfool (DF), %cite
%and the attacks from AA: APGD, FAB, SQR%cite
%. Natural Evolution Strategy (NES) is also formulated in the search space, but it is not included in the experiments because of the high computational cost. The detailed parameters are included in the supplement material. Attack $a$ is an instance from $\sA$, or $a \in \sA$. From the grammar rules, the result attack $s$ from the search space will be a sequence of attack containing various $a$ from $\sA$. 
%
%$D()$ is a decorator to the space $\sA$, and decorator is defined to be a modifier that is applicable to all the attacks. There are three parts in the decorator: randomize, EOT, and repeat. Randomize decorator takes a boolean whose value is True if any $a \in \sA$ has randomized component, and is False if it is deterministic. The attack decides the implementation of randomness, which can be whether to fix seed, or can be whether to start from the original image. EOT decorator takes value of $m \in \sZ^{+}$, and will make any query to the model execute $m$ times and then take the average. Repeat decorator takes value of $n \in \sZ^{+}$ and will repeat the attack $n$ times as a sequence of attack. In practice, repeat decorator is only meaningful if the randomize decorator is True. 


%\subsection{Loss Search Space}
%Loss functions defines the objective that the attack algorithm tries to minimize. Attack algorithms and the loss are considered as a pair. The Loss search space can be defined through grammar rules.
%
%\begin{enumerate}
%    \item $\sL \rightarrow Modifiers(Targeted((\sC), ntargets))$
%    \item $\sC \rightarrow CE|Hinge|DLR|L1|Logit Matching...$
%\end{enumerate}
%
%Loss function takes the prediction and the label as inputs and has the signature of $L:\sY, \sY -> \sR$. 
%
%$Targeted$ means to set the loss to a targeted loss or non-targeted loss, and usually the difference is the sign of the loss. If the loss is targeted loss, the targeted classes will be the highest $ntargets$ logits (or probability) with the clean prediction, and the attack will perform $ntargets$ of times in the manner of sequence of attack. $Modifiers$ are flexible customizable modifiers to the loss. The examples are: adding cross entropy operation before loss computation, and subtracting the targeted loss by the labeled class loss for DF. 
%
%In this work, the loss considered are cross entropy, hinge loss \cite{CandW}, Difference in Logit Ratio (DLR), L1 loss, and logit matching. The detailed parameters are listed in the supplement material. If an attack algorithm does not need loss function to perform (e.g. SQR), then the formulation still holds but there is no effect to the algorithm semantically. 


\subsection{Attack Search Space}

The attack search space is denoted as $\sS$ and an instance is denoted as as $s$. There are two parts for each attack, the attack algorithm $\sA$ and the loss function $\sL$. In addition, the common parts across different attacks and different loss functions are abstracted as decorators $D()$ and $D'()$ respectively. 

In the attack search space, not only single attacks but also sequences of attacks are included. The attacks in a sequence of attack are expected to complement each other to achieve higher ASR. The semantics of a sequence of attack $s$ is to evaluate the attacks in order and return the first adversarial sample found as shown in Algorithm \ref{alg:seq_attack}. Note that the order in the sequence of the attacks matters as it affects the return of the adversarial image. This notion of sequence of attack is the same as the notion of ensemble of attacks in \cite{croce2020reliable}. 

%\begin{algorithm}[tb]
%  \caption{Sequence of attacks}
%  \label{alg:seq_attack}
%\begin{algorithmic}
%  \STATE {\bfseries Input:} $g$, $\vx$, sequence attacks list $a$ with size n\; 
%  \STATE {\bfseries Output:} $\vx'$\;
%%   \REPEAT
%%   \STATE Initialize $noChange = true$.
%  \FOR{$i=1$ {\bfseries to} $n$}
%  	\STATE $\vx'$=$s[i](g, \vx)$\;
%    \IF{$C(\vx',g,y)$}
%      \STATE Return $\vx'$\;
%    \ENDIF
%    \ENDFOR
%  \STATE Return $\vx'$\;
%%   \UNTIL{$noChange$ is $true$}
%\end{algorithmic}
%\end{algorithm}

To further define syntax of $\sS$, we use the grammar rules. 

\begin{enumerate}
    \item $\sS \rightarrow \sS;\sS| (D(\sA), D'(\sL))$
    \item $D(\sA) \rightarrow Repeat(EOT(Randomize(\sA), m),n)$
    \item $\sA \rightarrow a=PGD(param)|DF(param)|FAB(param)|...$
    \item $D'(\sL) \rightarrow Modifiers(Targeted((\sL), ntargets))$
    \item $\sL \rightarrow l=CE|Hinge|DLR|L1|Logit Matching...$
\end{enumerate}

From the grammar rules, the result attack $s$ from the search space will be a sequence of algorithm and loss pairs $(a,l)$. 

$\sA$ is the space containing the attack algorithms along with the parameters. The algorithms include both the standard FGSM, PGD, C\&W, Deepfool (DF), %cite
and the attacks from AA: APGD, FAB, SQR%cite
. Natural Evolution Strategy (NES) is also formulated in the search space, but it is not included in the experiments because of the high computational cost. The detailed parameters are included in the supplement material. Attack $a \in \sA$ is a semantically defined attack which admits to the MA specification. 

$D()$ is the decorator to $\sA$ and there are three parts: randomize, EOT, and repeat. Randomize decorator takes a boolean whose value is True if any $a \in \sA$ has randomized component, and is False if it is deterministic. The attack decides the implementation of randomness, which can be whether to fix seed, or can be whether to start from the original image. EOT decorator executes $m$ times and then take the average. Repeat decorator repeats the attack $n$ times as a sequence of attack. In practice, repeat decorator is only meaningful if the randomize decorator is True. 

$\sL$ is the space of loss functions. The loss considered are cross entropy, hinge loss \cite{CandW}, Difference in Logit Ratio (DLR), L1 loss, and logit matching. The detailed parameters are listed in the supplement material. If an attack algorithm does not need loss function to perform (e.g. SQR), then the formulation still holds but there is no effect to the algorithm semantically.

$D'()$ is the decorator to $\sL$, and the two parts are $Modifiers$ and $Targeted$ . $Modifiers$ are flexible customizable modifiers to the loss. The examples are: the flag to add cross entropy operation before loss computation, and the flag to subtract the targeted loss by the labeled class loss in the targeted setting. $Targeted$ means to set the loss to a targeted loss or non-targeted loss, and usually the difference is the sign of the loss. If the loss is targeted loss, the targeted classes will be the highest $ntargets$ logits (or probability) with the clean prediction, and the attack will perform $ntargets$ times in the manner of sequence of attacks.


==> tables/attack_params.tex <==

\begin{table}[t]
\tra{1.15}
\centering
\caption{Hyperparameters of the attack search space.}
\label{attack_params}
\vskip 0.15in
{
\fontfamily{lmtt}\selectfont
\footnotesize
\begin{tabular}{@{}rcccl@{}}
\toprule
%    Name  & Description & Range & Log & Type & Attacks\\
%  \midrule
%  %\ding{51}
%step & number of steps & $[5,100]$ & - & int & PGD, NES \\  
%rel\_stepsize & the relative stepsize of the update & $[1/1000, 1]$ & \ding{51} & float & PGD, NES\\
%candidates & top number of logits to consider & $[2,10]$ & - & int & DF \\ 
%max\_iter & the max number of iterations & $[20, 200]$ & - & int & C\&W\\
%learning\_rate & learning rate for inner optimization & $[0.0001,0.01]$ & \ding{51} & float  & C\&W\\ 
%n\_samples & the number of samples for the estimation & $[400, 4000]$ & \ding{51} & int & NES \\
%rho & threshold of step size decrease & $[0.5, 0.9]$ & - & float & APGD\\
%n\_iter & number of iterations& $[10, 500]$ & - & int & APGD, FAB\\
%eta & overshooting & $[1, 1.2]$ & - & float & FAB \\
%beta & backward step & $[0.7, 1]$ & - & float & FAB \\
%n\_queries & number of queries & $[1000, 8000]$ & - & int & SQR \\
%p\_init & size of the squares & $[0.5, 0.9]$ & - & float & SQR \\

Name & Range & Log & Type & Attacks\\
\midrule
step & $[5,100]$ & - & int & PGD, NES \\  
rel\_stepsize & $[1/1000, 1]$ & \ding{51} & float & PGD, NES\\
candidates &  $[2,10]$ & - & int & DF \\ 
confidence & $[0,0.1]$ & - & float & C\&W \\
max\_iter & $[20, 200]$ & - & int & C\&W\\
learning\_rate & $[0.0001,0.01]$ & \ding{51} & float  & C\&W\\ 
n\_samples & $[400, 4000]$ & \ding{51} & int & NES \\
rho & $[0.5, 0.9]$ & - & float & APGD\\
n\_iter &  $[10, 500]$ & - & int & APGD, FAB\\
eta & $[1, 1.2]$ & - & float & FAB \\
beta &  $[0.7, 1]$ & - & float & FAB \\
n\_queries & $[1000, 8000]$ & - & int & SQR \\
p\_init & $[0.5, 0.9]$ & - & float & SQR \\

%  \multirow{3}{*}{FGSM} & Decorators: Random, *Repeat, EOT & $\sZ[1,1]$,$\sZ[10,10000]$, $\sZ[1,100]$ \\
%  & loss : loss function & ['ce', 'dlr'] \\
%  & set\_targeted: set objective to be multitargeted attack & $\sB$ \\
%  \hline
%  \multirow{5}{*}{PGD} & Decorators: Random, Repeat, EOT & $\sZ[1,1]$, $\sZ[1,10]$, $\sZ[1,20]$ \\
%  & loss: loss function & ['ce', 'dlr'] \\ 
%  & step: number of steps & $\sZ[5,100]$ \\ 
% *rel\_stepsize: the relative stepsize of the update & $\R[1/1000, 1]$ \\
%  & set\_targeted: set objective to be multitargeted attack & $\sB$ \\
%  \hline
%  \multirow{4}{*}{DF} & Decorators: Random, Repeat, EOT & $\sZ[0,0]$, $\sZ[1,1]$, $\sZ[1,1]$ \\
%  & loss : loss function & ['ce', 'softmax', 'dlr'] \\
%  & set\_targeted: set objective to be targeted attack & $\sB$ \\
%  & candidates: top number of logits to consider & $\sZ[2,10]$ \\
%  \hline
%  \multirow{4}{*}{C\&W} & Decorators: Random, Repeat, EOT & $\sZ[1,1]$, $\sZ[1,1]$, $\sZ[1,1]$ \\
%  & confidence: the confidence required & $\R[0,0.1]$ \\
%  & max\_iter: the max number of iterations & $\sZ[20, 200]$ \\
%  & *learning\_rate: learning rate for inner optimization & $\R[0.0001,0.01]$ \\
%  \hline
%  \multirow{4}{*}{NES} & Decorators: Random, Repeat, EOT & $\sZ[1,1]$, $\sZ[1,1]$, $\sZ[1, 1]$ \\
%  & step: number of steps & $\sZ[20, 80]$ \\
%  & *rel\_stepsize: the relative stepsize of the update & $\R[0.01, 0.1]$ \\
%  & *n\_samples: the number of samples for the estimation & $\sZ[400, 4000]$ \\
%  \hline
%  \multirow{4}{*}{APGD} & Decorators: Random, Repeat(n\_restart), EOT & $\sZ[1,1]$, $\sZ[1,10]$, $\sZ[1, 20]$ \\
%  & loss: loss function & ['ce', 'dlr'] \\ 
%  & rho: threshold of step size decrease & $\R[0.5, 0.9]$ \\
%  & n\_iter: number of iterations& $\sZ[20, 500]$ \\
%  \hline
%  \multirow{4}{*}{FAB} & Decorators: Random, Repeat(n\_restart), EOT & $\sZ[1,1]$, $\sZ[1,40]$, $\sZ[1, 1]$ \\
%  & n\_iter: number of iterations & $\sZ[10, 200]$ \\
%  & eta: overshooting & $\R[1, 1.2]$ \\
%  & beta: backward step & $\R[0.7, 1]$ \\
%  \hline
%  \multirow{4}{*}{SQR} & Decorators: Random, Repeat(n\_restarts), EOT & $\sZ[1,1]$, $\sZ[1,3]$, $\sZ[1, 1]$ \\
%  & n\_queries: number of queries & $\sZ[1000, 8000]$ \\
%  & p\_init: parameter to control size of squares & $\R[0.5, 0.9]$ \\
%  & loss: loss function & ['ce', 'margin'] \\
  \bottomrule
\end{tabular}
}
\vskip -0.1in
\end{table}


==> tables/bm_result_explanation.tex <==

\begin{table}[t]
\caption{List of models where MA has much better evaluation than AA. Transformation refers to the network transformation used, attack refers to the first attack algorithm of the search, and loss refers to the first loss of the search}
\label{bm_result_explanation}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccr}
\toprule
 Net & Transformation & Attack & Loss \\
\midrule
a5& - & FAB & ce-U \\
a6& - & PGD & hinge-U \\
a9& - & APGD & hinge-U \\
a10$*$ & - & NES & ce-U \\
b5&	- & SQR & hinge-U \\
b10& Removal & APGD & hinge-T \\
b11& - & PGD & hinge-T \\
b12& - & APGD & L1-U \\
b13& - & APGD & dlr-T \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/bm_results.tex <==

%\begin{table}[t]
%\caption{Comparison between results of AA and Searched attacks (including AA attacks in the search space). The result is measured in Robustness(\%). The threat model is 4/255 Linf norm on CIFAR10 dataset. (t) means the time for the attack, and (tt) means the total time used including the search. All time is measured in seconds. In A10$*$ experiment, NES algorithm into the search space and it is selected as the expensive effective attack. }
%\label{bm1_result}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccccr}
%\toprule
% & AA & MA & AA(t) & MA(t) & MA(tt) \\
%\midrule
%a1& 1.09&  1.07&	110&	311&	3592\\
%a2& 44.78&	44.69&	1467&	1166&	5868\\
%a3& 2.29&	1.96&	481&	402&	5983\\
%a4& 0.83&	0.11&	350&	116&	1630\\
%a5& 75.93&	\textbf{3.04}&	105&	745&	5563\\
%a6& 22.19&	\textbf{13.14}&	1136&	1000&	6906\\
%a7& 4.49&	3.96&	1660&	2820&	13399\\
%a8& 2.85&	2.71&	194&	239&	3978\\
%a9& 19.82&	\textbf{11.11}&	2892&	1266&	12651\\
%a10& 64.91&	63.56&	9416&	11502&	26861\\
%a10$*$ & 64.91 & \textbf{17.70}& 9416&  136800 & 229680\\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}


%\begin{table}[t]
%\caption{Comparison between results of AA and Searched attacks (including AA attacks in the search space). The type of defenses are presented in table ... The threat model is 8/255 Linf norm on CIFAR10 dataset. To be consistent with the literature, the result is measured in empirical robustness(\%). (t) means the time for the attack, and (tt) means the total time used including the search. All time is measured in minutes. }
%\label{bm2_result}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccccr}
%\toprule
% & AA & MA & AA(t) & MA(t) & MA(tt) \\
%\midrule
%b1&	 60.05&	60.01&  706&	255&	945 \\
%b2&	 56.16&	56.18&  801&	145&	822 \\
%b3&	 36.74&	37.11&	381&    302&	1028 \\
%b4&	 5.15&	5.23&   107&	124&	785 \\
%b5&	 5.40&	\textbf{2.75}&  95& 	169&	1016 \\
%b6&	 50.84&	50.81&	734&	372&	1127 \\
%b7&	 50.94&	50.89&	742&	486&	1293 \\
%b8&	 57.19&	57.16&  671&	429&	1120 \\
%b9&	 60.72&	60.33&	621&	140&	772 \\
%b10& 15.27&	\textbf{5.24}&	261&	79&		825 \\
%b11& 49.53&	\textbf{41.99}&	255&	462&	1362 \\
%b12& 22.29&	\textbf{13.45}&	114&	374&	1397 \\
%b13& 42.72& \textbf{2.79} & 5  &    4  &	279 \\
%b14& 90.40& \textbf{44.88}& 7&    34 & 125 \\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}

==> tables/defense_list.tex <==


%\begin{table}[t]
%\centering
%\caption{List of network and defences. Conv means a four layered CNN. The model with * means the network is available from authors, models are retrained otherwise. The model with - means the network has non-differentiable component. All the models are available, and the detailed parameters are in the repository. }
%\label{defense_list}
%\vskip 0.15in
%{
%%\fontfamily{lmtt}\selectfont
%\footnotesize
%\begin{tabular}{ll}
%\toprule
% & Defense \\
%\midrule
%a1& None\\
%a2&	Adversarial Training \cite{madry2017towards}\\
%a3$^\dagger$& Thermometer Encoding \cite{buckman2018thermometer}\\
%\multirow{2}{*}{a4$^\dagger$}&  JPEG \cite{das2017keeping} + \\
%& Reverse Sigmoid \cite{lee2018defending}\\
%a5& Feature Detector  \cite{metzen2017detecting} \\
%a6& Input Random Rotation \cite{eriba2019kornia} \\
%a7$^\dagger$& Ensemble \cite{pang2019improving} \\
%a8& Defensive Distillation \cite{DBLP:journals/corr/PapernotMWJS15}\\
%a9& kWTA 0.1 no Adv \cite{xiao2019resisting} \\
%a10& kWTA 0.1 Adv \cite{xiao2019resisting}\\
%b1$^*$&  AWP\_RST \cite{wu2020adversarial}\\
%b2$^*$&  AWP\_TRADES \cite{wu2020adversarial}\\
%b3$^*$&  Feature Scatter \cite{feature_scatter} \\
%b4&	 JEM \cite{grathwohl2020classifier} \\
%b5&	 kWTA 0.1 Adv \cite{xiao2019resisting} \\
%b6&	 Ensemble Resnet \cite{wang2019resnets} \\
%b7$^*$&  MART \cite{Wang2020Improving} \\
%b8$^*$&  HYDRA \cite{sehwag2020hydra} \\
%b9$^\dagger$&  b1 + JPEG + Reverse Sigmoid \\
%b10$^\dagger$& b4 + JPEG + Reverse Sigmoid \\
%b11& b1 + Random Rotation \\
%b12& b4 + Random Rotation \\
%b13& Turning Weakness into Strength \cite{Yu_2019_NeurIPSweakness} \\
%b14& CCAT \cite{stutz2020confidencecalibrated} \\
%\bottomrule
%\multicolumn{2}{l}{$^\dagger$ model with non-differentiable components}\\
%\multicolumn{2}{l}{$^*$ model obtained from the authors}\\
%
%\end{tabular}
%}
%\vskip -0.1in
%\end{table}

==> tables/parameter_settings.tex <==

%\begin{table}[t]
%\caption{Default search parameter setting for the search}
%\label{parameters}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lr}
%\toprule
%parameter & value \\
%\midrule
%Max attacks & 3 \\
%Number of base samples & 100 \\
%Number of trials & 64 \\
%SHA sample multiply factor ($k$) & 2 \\
%SHA trial division factor ($\tau$) & 4 \\
%Search algorithm & TPE \\
%Enable BPDA search for AA & $\surd$ \\
%Enable BPDA search for MA & $\surd$ \\
%Enable removal search for AA & $\times$ \\
%Enable removal search for MA & $\surd$ \\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}
